Quantum Data Management: From Theory to Opportunities

Quantum computing has emerged as a transformative tool for future data management. Classical problems in database domains, including query optimization, data integration, and transaction management, have recently been addressed using quantum computing techniques. This tutorial aims to establish the theoretical foundation essential for enhancing methodologies and practical implementations in this line of research. Moreover, this tutorial takes a forward-looking approach by delving into recent strides in quantum internet technologies and the nonlocality theory. We aim to shed light on the uncharted territory of future data systems tailored for the quantum internet.

==> algorithms/autofeat.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[t]
\footnotesize
\SetAlgoLined
\caption{Feature Discovery}
\label{alg:autofeat}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{// }{}
\SetKw{KwBy}{by}
\SetKwFunction{KwFn}{Function}
\SetKwProg{Fn}{Function}{ is}{end}
\Input{queue $Q$ containing the base table $T_0$, $R_{sel}$ selected features from $T_0$, $\tau$ null value ratio threshold, $\kappa$ maximum number of features to select from a table }
\Output{dictionary of paths with scores $rank$ }
\BlankLine
% \bf Initialization:
\Fn{autofeat(Q, P=None)}{ 
\tcp{Previous queue initialisation}
$ P = Q $ \\

\While {Q} {
    $T_0 = pop(Q)$ \\ 
    $neighbours = get\_neighbours(T_0)$ \\ 

    \ForEach {node $T_n \in neighbours$} {
        $join\_keys = get\_join\_keys(T_0, T_n)$ \\
        $C = {}$ empty queue \\ 

        \While {P} {
            \ForEach{join key $jk \in join\_keys$} {
                $R = join(T_0, T_n, jk)$ \\ 
                \If{$R$ is not possible} {
                    $ continue $ \\
                }

                $D = get\_data\_quality(R)$ \\ 
                \If{$D < \tau $ } {
                    $ continue $ \\
                }

                $R_{rel}, score_{rel} = measure\_relevance(R, \kappa)$\\ 
                \If{$R_{rel}$ is empty } {
                \tcp{Save the current join path}
                    $update(C, R)$ \\ 
                    $ continue $ \\
                }

                $R_{red}, score_{red} = measure\_redundancy(R[R_{rel}], R_{sel})$ \\ 
                \If{$R_{red}$ is empty  } {
                    \tcp{Save the current join path}
                    $update(C, R)$ \\ 
                    $ continue $ \\
                }
                
                $R_{sel} = R_{sel} \cup R_{red} $ \\ 
                $score = compute\_score(score_{rel}, score_{red})$ \\ 
                $rank_n = (score, R)$ \\  

                \tcp{Update current queue, C, with the join, R}
                $update(C, R)$ \\ 
            }
            $update(P, C)$ \\ 
        } 
    }

} 

$autofeat(neighbours, P)$ \\ 


}
\end{algorithm}


==> algorithms/ranking_score.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[tb]
\footnotesize
\SetAlgoLined
\caption{Ranking score}
\label{alg:ranking}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{// }{}
\SetKw{KwBy}{by}
\SetKwFunction{KwFn}{Function}
\SetKwProg{Fn}{Function}{ is}{end}
\Input{$score_{rel}$ the scores from the relevance analysis, $score_{red}$ the scores from the redundancy analysis}
\Output{$ranking\_score$ one score number}
\BlankLine
% \bf Initialization:
\Fn{compute\_score($score_{rel}$, $score_{red}$)}{ 

$N_{rel} = length(score_{rel})$ \\ 
$N_{red} = length(score_{red})$ \\ 
$sum_{rel} = sum(score_{rel}) / N_{rel}$ \\ 
$sum_{red} = sum(score_{red}) / N_{red}$ \\ 
$ranking\_score = (N_{red} * sum_{rel} + N_{rel} * sum_{red}) / (N_{rel} * N_{red}) $ 
}
\end{algorithm}

